PHANGS: Constraining Star Formation Timescales Using the Spatial Correlations of Star Clusters and Giant Molecular Clouds

In the hierarchical view of star formation, giant molecular gas clouds (GMCs) undergo fragmentation to form small-scale structures made up of stars and star clusters. Here we study the connection between young star clusters and cold gas across a range of extragalactic environments by combining the high resolution (1") PHANGS-ALMA catalogue of GMCs with the star cluster catalogues from PHANGS-HST. The star clusters are spatially matched with the GMCs across a sample of 11 nearby star-forming galaxies with a range of galactic environments (centres, bars, spiral arms, etc.). We find that after 4-6 Myr the star clusters are no longer associated with any gas clouds. Additionally, we measure the autocorrelation of the star clusters and GMCs as well as their cross-correlation to quantify the fractal nature of hierarchical star formation. Young ($\leq$ 10 Myr) star clusters are more strongly autocorrelated on kpc and smaller spatial scales than the >10 Myr stellar populations, indicating that the hierarchical structure dissolves over time.

==> tables/table_ccf_plaw.tex <==
\begin{table*}
\sisetup{separate-uncertainty,table-auto-round=true,round-mode=places,round-precision=2}
\centerline{Table 5. Best-Fitting Power Law Slope $\alpha$ for the Cross-correlation Functions}
\begin{tabular}{l S[table-figures-integer=1, table-figures-decimal=2] S[table-figures-integer=1, table-figures-decimal=2] S[table-figures-integer=1, table-figures-decimal=2] S[table-figures-integer=1, table-figures-decimal=2]}
\hline\hline
\mcone{Galaxy} & \multicolumn{1}{r}{All SCs} & \multicolumn{1}{r}{SCs $\leq10$ Myr} & \multicolumn{1}{r}{SCs $>10$ Myr} \\
\hline
NGC~0628 & -0.14 \pm 0.02 & -0.08 \pm 0.05 & -0.03 \pm 0.01 \\
NGC~1365 & -0.12 \pm 0.08 & -0.23 \pm 0.06 & -0.13 \pm 0.08 \\
NGC~1433 & -0.31 \pm 0.06 & -0.33 \pm 0.05 & -0.17 \pm 0.07 \\
NGC~1559 & -0.11 \pm 0.04 & -0.52 \pm 0.12 & -0.08 \pm 0.05 \\
NGC~1566 & -0.10 \pm 0.01 & -0.23 \pm 0.02 & -0.02 \pm 0.03 \\
NGC~1792 & -0.14 \pm 0.04 & -0.13 \pm 0.05 & -0.19 \pm 0.04 \\
NGC~3351 & -0.34 \pm 0.07 & -0.20 \pm 0.10 & -0.13 \pm 0.04 \\
NGC~3627 & -0.07 \pm 0.03 & -0.14 \pm 0.04 & -0.06 \pm 0.03 \\
NGC~4535 & -0.25 \pm 0.03 & -0.34 \pm 0.02 & -0.13 \pm 0.07 \\
NGC~4548 & -0.27 \pm 0.09 & -0.46 \pm 0.05 & -0.04 \pm 0.08 \\
NGC~4571 & -0.23 \pm 0.04 & -0.22 \pm 0.06 & -0.12 \pm 0.04 \\
\hline
\end{tabular}
\caption{A Levenberg--Marquardt non-linear least squares minimization is used to fit a power-law of the form $A\theta^{\alpha}$ to the autocorrelation functions shown in Figure~\ref{fig:cross_grid}.}
\label{tab:ccf_plaw}
\end{table*}
